Optimal and Approximate Q-value Functions for Decentralized POMDPs

Decision-theoretic planning is a popular approach to sequential decision making problems, because it treats uncertainty in sensing and acting in a principled way. In single-agent frameworks like MDPs and POMDPs, planning can be carried out by resorting to Q-value functions: an optimal Q-value function Q* is computed in a recursive manner by dynamic programming, and then an optimal policy is extracted from Q*. In this paper we study whether similar Q-value functions can be defined for decentralized POMDP models (Dec-POMDPs), and how policies can be extracted from such value functions. We define two forms of the optimal Q-value function for Dec-POMDPs: one that gives a normative description as the Q-value function of an optimal pure joint policy and another one that is sequentially rational and thus gives a recipe for computation. This computation, however, is infeasible for all but the smallest problems. Therefore, we analyze various approximate Q-value functions that allow for efficient computation. We describe how they relate, and we prove that they all provide an upper bound to the optimal Q-value function Q*. Finally, unifying some previous approaches for solving Dec-POMDPs, we describe a family of algorithms for extracting policies from such Q-value functions, and perform an experimental evaluation on existing test problems, including a new firefighting benchmark problem.

==> Makefile <==
################################ MACROS ################################
#
# DOC: the document
# FIG: directory for figures
# BIB: bibliography database
# BST: bibliography style
# SEL: selected pages; e.g., "odd", "even", "2\:4,6"
#
#DOC = jp_QV4Dec-POMDPs
DOC = oliehoek08a
FIG = figs
BIB = 
BST =
SEL = ""
 
############################### PROGRAMS ###############################
#
TEX = latex
BIBTEX = bibtex
DVISELECT = dviselect
INDEX = makeindex
DVIPS = dvips -t letter -Ppdf -G0

# changing prepress to screen produces much smaller files (but prepress is better for beamer)
PS2PDF = ps2pdf -sPAPERSIZE=letter -dPDFSETTINGS=/prepress -dEmbedAllFonts=true -dEncodeGrayImages=false -dEncodeMonoImages=false -dEncodeColorImages=false 
# PS2PDF = ps2pdf -dPDFSETTINGS=/screen -dEmbedAllFonts=true -dEncodeGrayImages=true -dAutoFilterGrayImages=false -dGrayImageFilter=/FlateEncode \
#        -dEncodeMonoImages=true -dAutoFilterMonoImages=false -dMonoImageFilter=/FlateEncode \
#        -dEncodeColorImages=true -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode

DVILJ4 = dvilj4mak
XDVI = xdvi -expert -hush -s 6 -geometry -0+0
#XPS = ghostview -watch -geometry -0+0
XPS = gview
XPDF = acroread 
PRINT = lpr -Plaser1
MAKE = make
RM = rm -f
 
############################ Inference Rules ###########################
#
.SUFFIXES: .tex .dvi .ps .lj .aux .bbl .pdf .idx .ind
.tex.dvi:
	( \
	$(TEX) $<; \
	while \grep -q "Rerun to get cross-references right." $(<:.tex=.log); \
	do \
		\latex $<; \
	done \
	)
.dvi.ps:
	$(DVIPS) -o $@ $< 
.dvi.lj:
	$(DVILJ4) $<
.tex.aux:
	$(TEX) $<
.aux.bbl:
	$(BIBTEX) $*
.ps.pdf:
	$(PS2PDF) $<
.idx.ind:
	${INDEX} $<
	${TEX} ${DOC}.tex

################################# Rules ################################
#
all:    dvi
 
aux:    $(DOC).aux
bib:    $(DOC).bbl
index:	$(DOC).ind
 
dvi:    $(DOC).dvi
dvisel: $(DOC)-$(SEL).dvi
ps: $(DOC).ps
pssel:  $(DOC)-$(SEL).ps
lj: $(DOC).lj
ljsel:  $(DOC)-$(SEL).lj

pdf:	$(DOC).pdf

xdvi:   $(DOC).dvi
	$(XDVI) $<
xsel:   $(DOC)-$(SEL).dvi
	$(XDVI) $<
xps:    $(DOC).ps
	$(XPS) $<
xpdf:    $(DOC).pdf
	$(XPDF) $<
xpssel: $(DOC)-$(SEL).ps
	$(XPS) $<
 
print:  $(DOC).ps
	$(PRINT) $<
prsel:  $(DOC)-$(SEL).ps
	$(PRINT) $<
 
$(DOC)-$(SEL).dvi: $(DOC).dvi
	$(DVISELECT) $(SEL) $< $@
 
fig:
	@cd $(FIG); $(MAKE) DIR=$(FIG)
 
new:
	$(RM) $(DOC).dvi

clean:
	$(RM) $(DOC).aux $(DOC).log ${DOC}.brf
	$(RM) $(DOC).toc $(DOC).lot $(DOC).lof
	$(RM) $(DOC).ttt $(DOC).lot $(DOC).fff
	$(RM) $(DOC).blg $(DOC).out
	$(RM) $(DOC).dvi $(DOC)-*.dvi
	$(RM) $(DOC).ps $(DOC)-*.ps
	$(RM) $(DOC).pdf
	$(RM) texput.log core
 
distclean: clean
	cd $(FIG); $(MAKE) clean
 
bak:
	bakdir="./BAK/`date  --iso-8601=minutes`"; \
	test ! -d $$bakdir && mkdir -p $$bakdir; \
	cp -f *.tex $$bakdir


==> tables/MAAstarFF242.tex <==
\begin{table}
  \newcommand{\hhhhline}{\hhline{|~~|----|}}
  \centering
  \begin{tabular}{|ccrrrr|}
    \hline
    $h$&$V^*$&&$n_\partJPol$
    %&$n_P$
    &$T_\GMAA$&$T_Q$\\
    \hline
%     \hline
%     \multirow{3}{*}{1}&\multirow{3}{*}{
%       $-1.7000$ % HORIZON 1
%     }
%      &$\QMDP$&
%     $16$ & $0$ & $\zeros$ s& $\zeros$ s\\
%     \hhhhline
%     &&$\QPOMDP$&
%     $16$ & $0$ & $\zeros$ s& $\zeros$ s\\
%     \hhhhline
%     &&$\QBG$&
%     $16$ & $0$ & $\zeros$ s& $\zeros$ s\\
%     \hline
%     \hline
%     \multirow{3}{*}{2}&\multirow{3}{*}{
%       $-3.0576$ % HORIZON 2
%     }
%      &$\QMDP$&
%     $2,576$ & $16$ & $0.02$ s& $0.71$ s\\
%     \hhhhline
%     &&$\QPOMDP$&
%     $31$ & $16$ & $\zeros$ s& $0.02$ s\\
%     \hhhhline
%     &&$\QBG$&
%     $31$ & $16$ & $\zeros$ s& $0.03$ s\\
%     \hline
    \hline
    \multirow{3}{*}{3}&\multirow{3}{*}{
      $-3.8312$ % HORIZON 3
    }
     &$\QMDP$&
    $1,050,128$
    %& $1,546$
    & $2.99$ s& $1.41$ s\\
    \hhhhline
    &&$\QPOMDP$&
    $176,480$ 
    % & $1,036$
    & $0.49$ s& $0.98$ s\\
    \hhhhline
    &&$\QBG$&
    $176,480$ 
    % & $1,036$
    & $0.50$ s& $1.61$ s\\
    \hline
    \hline
    \multirow{3}{*}{4}&\multirow{3}{*}{
      $-4.4409$ % HORIZON 4
    }
     &$\QMDP$&
    $$ 
    % & $$
    & $$ s& $2.14$ s\\
    \hhhhline
    &&$\QPOMDP$&
    $17,180,394,512$ % (was $525,328$)
    % & ???? $525,316$
    & $187,542$ s& $62.86$ s\\
    \hhhhline
    &&$\QBG$&
    $17,180,394,512$ % (was $525,328$) 
    %& ???? $393,991$
    & $192,578$ s& $103.27$ s\\
    \hline

  \end{tabular}
  \caption{$\MAA$ results for Fire Fighting $\langle n_h=4, n_f=2 \rangle$.}
  \label{tab:MAAstarFF242}
\end{table}


==> tables/MAAstarFF243.tex <==
\begin{table}
  \newcommand{\hhhhline}{\hhline{|~~|----|}}
  \centering
  \begin{tabular}{|ccrrrr|}
    \hline
    $h$&$V^*$&&$n_\partJPol$
    %&$n_P$
    &$T_\GMAA$&$T_Q$\\
    \hline
%     \hline
%     \multirow{3}{*}{1}&\multirow{3}{*}{
%       $-3.9407$ % HORIZON 1
%     }
%      &$\QMDP$&
%     $16$ & $0$ & $\zeros$ s& $0.01$ s\\
%     \hhhhline
%     &&$\QPOMDP$&
%     $16$ & $0$ & $\zeros$ s& $\zeros$ s\\
%     \hhhhline
%     &&$\QBG$&
%     $16$ & $0$ & $\zeros$ s& $\zeros$ s\\
%     \hline
%     \hline
%     \multirow{3}{*}{2}&\multirow{3}{*}{
%       $-7.7065$ % HORIZON 2
%     }
%      &$\QMDP$&
%     $3,088$ & $16$ & $0.10$ s& $17.94$ s\\
%     \hhhhline
%     &&$\QPOMDP$&
%     $528$ & $16$ & $\zeros$ s& $0.09$ s\\
%     \hhhhline
%     &&$\QBG$&
%     $104$ & $16$ & $\zeros$ s& $0.18$ s\\
%     \hline
    \hline
    \multirow{3}{*}{3}&\multirow{3}{*}{
      $-11.1356$ % HORIZON 3
    }
     &$\QMDP$&
    $42,995,216$
    %& $3,586$
    & $142.95$ s& $35.97$ s\\
    \hhhhline
    &&$\QPOMDP$&
    $197,136$
    % & $526$
    & $0.57$ s& $5.79$ s\\
    \hhhhline
    &&$\QBG$&
    $65,808$
    % & $271$
    & $0.19$ s& $10.78$ s\\
    \hline
    \hline
    \multirow{3}{*}{4}&\multirow{3}{*}{
      $-14.1068$ % HORIZON 4
    }
     &$\QMDP$&
    $$ 
    % & $$ 
    & $$ s& $53.81$ s\\
    \hhhhline
    &&$\QPOMDP$&
    $17,180,197,648$ % (was $328,464$)
    % & ???? $196,608$
    & $185,796$ s& $370.08$ s\\
    \hhhhline
    &&$\QBG$&
    $17,180,000,784$ % (was $131,600$) 
    %& ???? $65,806$
    & $191,428$ s& $690.23$ s\\
    \hline

  \end{tabular}
  \caption{$\MAA$ results for Fire Fighting $\langle n_h=4, n_f=3 \rangle$.}
  \label{tab:MAAstarFF243}
\end{table}


==> tables/MAAstartemplate.tex <==
\begin{table}
  \newcommand{\hhhhline}{\hhline{|~~|----|}}
  \centering
  \begin{tabular}{|ccrrrr|}
    \hline
    $h$&$V^*$&&$n_\partJPol$
    %&$n_P$
    &$T_\GMAA$&$T_Q$\\
    \hline
    \hline
    \multirow{3}{*}{1}&\multirow{3}{*}{
      $$ % HORIZON 1
    }
     &$\QMDP$&
    $$ & $$ & $$ s& $$ s\\
    \hhline{|~~|-----|}
    &&$\QPOMDP$&
    $$ & $$ & $$ s& $$ s\\
    \hhline{|~~|-----|}
    &&$\QBG$&
    $$ & $$ & $$ s& $$ s\\
    \hline
    \hline
    \multirow{3}{*}{2}&\multirow{3}{*}{
      $$ % HORIZON 2
    }
     &$\QMDP$&
    $$ & $$ & $$ s& $$ s\\
    \hhline{|~~|-----|}
    &&$\QPOMDP$&
    $$ & $$ & $$ s& $$ s\\
    \hhline{|~~|-----|}
    &&$\QBG$&
    $$ & $$ & $$ s& $$ s\\
    \hline
    \hline
    \multirow{3}{*}{3}&\multirow{3}{*}{
      $$ % HORIZON 3
    }
     &$\QMDP$&
    $$ & $$ & $$ s& $$ s\\
    \hhline{|~~|-----|}
    &&$\QPOMDP$&
    $$ & $$ & $$ s& $$ s\\
    \hhline{|~~|-----|}
    &&$\QBG$&
    $$ & $$ & $$ s& $$ s\\
    \hline
    \hline
    \multirow{3}{*}{4}&\multirow{3}{*}{
      $$ % HORIZON 4
    }
     &$\QMDP$&
    $$ & $$ & $$ s& $$ s\\
    \hhline{|~~|-----|}
    &&$\QPOMDP$&
    $$ & $$ & $$ s& $$ s\\
    \hhline{|~~|-----|}
    &&$\QBG$&
    $$ & $$ & $$ s& $$ s\\
    \hline

  \end{tabular}
  \caption{$\MAA$ results for PROBLEM.}
  \label{tab:MAAstartemplate}
\end{table}

